Efficient Network Function Backup by Update Piggybacking

Network Function Virtualization (NFV) and Service Function Chaining (SFC) have been widely used to enable flexible and agile network management. To enhance reliability, some research has proposed to deploy backup function instances for prompt recovery when a primary instance fails. While most of the recent studies focus on speeding up recovery, less attention has been paid to the problem of minimizing the state update cost. In this work, we present PiggyBackup (Piggyback-based Backup), an efficient backup instance deployment and update protocol. Our key idea is to reuse the existing service chains traversing through servers in a network to help piggyback the update information. By doing this, we eliminate the header overhead and reduce the amount of update traffic significantly. To realize such a piggyback-based update more efficiently, we investigate the backup instance deployment and chain selection problems to enhance piggybacking opportunities and reduce the forwarding hop counts with explicit consideration of the distribution of service chains. Our simulation results show that PiggyBackup reduces the average overall update overhead by 47.65% and 39.56%, respectively, in a fat-tree topology as compared to random deployment and shortest path based deployment.

==> evaluation-1.tex <==

\ifx\isthesis\undefined
        \begin{table}[t] 
		\small
		\caption{Default simulation Setups}
		%\vspace{5mm}
		\centering  \label{tab:Parameter}
		\begin{tabular}{ll}
			\toprule
			       Parameter         & Values  \\ 
			\toprule
					Number of servers &20\\
			       Number of function types      & 20 \\
			       Number of chains      & 50 \\
			       Primary capacity per server & 8 \\
			       Backup capacity per server & 3 \\
				   Backup-primary association limit ($K$) & 5\\
			 \bottomrule
		\end{tabular}
		\label{tb:setting}
\end{table}
\else
%\afterpage{
%    \vspace*{\fill}{
        \begin{table}[t] 
		\small
		\caption{List of Settings}
		%\vspace{5mm}
		\centering  \label{tab:Parameter}
		\begin{tabular}{ll}
			\toprule
			       Parameter         & Default configuration  \\ 
			\toprule
					Number of servers &20\\
			       Number of function types      & 20 \\
			       Number of chains      & 50 \\
			       Primary capacity per server& 8 \\
			       Backup capacity per server & 3 \\
				   Backup-primary association limit ($K$) & 5\\
			 \bottomrule
		\end{tabular}
		\label{tb:setting}
\end{table}
%    }
%    \vspace*{\fill}
%    \clearpage
%}
\fi


\secc{Performance Evaluation}\label{sec:results}
We conduct extensive simulations to evaluate the performance of \name\
in a fat tree topology~\cite{AlFares2008}, which has been widely used
in many data center networks. We deploy a 4-pods fat tree, which
consists of 16 hosts and three layers of switches, i.e., 8 edge
switches, 8 aggregation switches and 4 core switches.  Each switch
connects to a physical machine, which installs a number of VMs.
Without otherwise stated, the default number of function types and
chains are set to 20 and 50, respectively, and the maximal number of
primary instances and backup instances that can be installed in a
server (i.e., server capacity) is 8 and 3, respectively.  We assign
each primary instance to a randomly-selected physical machine. For
each function type, we randomly deploy a roughly equal number of
instances in the network until the capacity of all the servers has
been fully utilized. Each backup instance can be associated with up to
$K=5$ primary instances by default.  The packet size of each piggyback
update and stand-alone update, respectively, is set to 20 and 60
bytes.  The default parameter settings are summarized in
Table~\ref{tb:setting}.
%\del{\textblue{The default parameter settings are summarized in



\ifx\isthesis\undefined
\begin{figure*}[t]
	\centering
	\begin{tabular}{ccc}
		\hspace{-12pt}
		\epsfig{width=2.25in,file=Impact_of_Backup_Capacity_10.eps}&
		\hspace{-10pt}
		\epsfig{width=2.25in,file=Impact_of_Backup_Capacity_20.eps}&
		\hspace{-10pt}
		\epsfig{width=2.25in,file=Impact_of_Backup_Capacity_30.eps}\\
		\footnotesize{(a) 10 chains}&
		\footnotesize{(b) 20 chains }&
		\footnotesize{(c) 30 chains }
	\end{tabular}
	\caption{Impact of backup capacity}
	\label{fig:capacity}
\end{figure*}
\else
%\afterpage{
	\vspace*{\fill}{
		\begin{figure}[ht]
			\centering
			\begin{tabular}{c}
				\epsfig{width=4in,file=Impact_of_Backup_Capacity_10.eps}\\
				\footnotesize{(a) 10 chains}\\
				\\
				\epsfig{width=4in,file=Impact_of_Backup_Capacity_20.eps}\\
				\footnotesize{(b) 20 chains }\\
				\\
				\epsfig{width=4in,file=Impact_of_Backup_Capacity_30.eps}\\
				\footnotesize{(c) 30 chains }
			\end{tabular}
			\caption{Impact of backup capacity}
			\label{fig:capacity}
		\end{figure}
	}
	\vspace*{\fill}
	%\clearpage
%}
\fi

We generate a set of chains, each of which is from a random
originating host to a random destination host and requests a sequence
of NFs randomly selected from a set of function types $\mathcal{F}$.
The length of a chain is also picked randomly, varying from 1 to 20.
We leverage a simple closest instance assignment scheme to assign
primary instances to a chain. That is, for a chain requesting NF
$f_i\rightarrow f_{i+1}$ in steps $i$ and $i+1$, the instance of $f_i$
will forward this chain to the closest instance of $f_{i+1}$. The
traffic arrival pattern of each chain follows a Poisson process with
the mean arrival rate of 1 packet per millisecond. Since our goal is
to demonstrate the benefit of reusing SFCs, the primary instance
assignment for SFCs should not affect the performance much.

We compare \name\ with two baseline algorithms: {\em i) random
placement}, which deploys backup instances in randomly selected
servers without considering the locations of primary instances, and
{\em ii) shortest path based placement:} primary instances
sequentially pick the closest available servers to deploy (or reuse)
their backup instances, while the selection order of primary instances
is determined randomly.  Our evaluation will examine the impact of
number of chains, the impact of server capacity, the impact of
backup-primary association limit, the effectiveness of chain
selection, and the performance of stand-alone backup instance
placement.

\ifx\isthesis\undefined
        \begin{figure}[t]
	        \centering
		    \epsfig{width=2.7in,file=Percentage_of_Piggybacked_Functions_zoom.eps}
	        \caption{Impact of number of chains and backup capacity}
	        \label{fig:chain-cap}
        \end{figure}
\else
%
\fi

\subsecc{Impact of Number of Chains}%Fig 4,5,6
We first check the percentage of primary instances whose backup can be
piggybacked in the three comparison schemes.
Fig.~\ref{fig:chainNum}(a) shows the results when the number of chains
varies from 10 to 50. The figure shows that, as the number of chains
increases, the opportunities of piggybacking grow accordingly,
matching the intuition of our design.  Since our design explicitly
considers the locations of primary instances and the traversing paths
of chains, we can fully utilize the piggybacking opportunities and
obtain almost 100\% of piggybackable instances. However, random
placement and shortest path based deployment would underutilize the
opportunities as they do not consider the routing of chains.

Fig. \ref{fig:chainNum}(b) demonstrates the piggybacking hop counts of
the comparison methods. The results show that random placement does
not consider the locations of primary instances and, thus, lead to long
piggybacking paths.  Shortest path based placement achieves the minimal
piggybacking hop counts since it always deploys the backup instances
nearby the primary instances. However, as shown in
Fig.~\ref{fig:chainNum}(a), it supports piggybacking for only
40\%--60\% of primary instances. Hence, those non-piggybackable
instances still need to use stand-alone packets to deliver updates, as
a result increasing the overall cost. By contrast, \name\ allows
almost all the primary instances to piggyback their updates, through a
slightly longer path.

We then plot in Fig.~\ref{fig:chainNum}(c) the total number of update
bytes, including piggybacking and stand-alone packets, of the three
methods. The results verify that shortest path based placement sends
stand-alone updates for a large proportion of primary instances and,
overall, produces a significantly higher update overhead.  Though our
piggybacking updates traverse through slightly longer paths, the
average overall overhead can still be reduced by 39.56\%, as compared
to shortest path based placement, since we fully utilize piggybacking
opportunities and minimize the stand-alone update cost. 




\subsecc{Impact of Server Capacity}%Fig 4,5,6
In this simulation, we examine the impact of backup capacity of each
server.  Figs.~\ref{fig:capacity}(a,b,c) illustrate the percentage of
piggybackable instances as the network includes 10, 20, and 30 chains,
respectively. For each figure, we plot the results when the backup
capacity varies from 2 to 6.  The results show that, when the backup
capacity increases, the piggybacking opportunities grow accordingly.
The percentage converges when the backup capacity increases to 4,
showing that a finite backup capacity can already ensure full
piggybacking updates. When the backup capacity is large enough, the
performance of various numbers of chains becomes indifferent. This
explains that, when a system supports sufficient backup capacity, even
a small number of chains can already realize the benefits of
piggybacking.

\ifx\isthesis\undefined
        \begin{figure}[t]
	        \centering
		    \epsfig{width=2.7in,file=Impact_of_Number_of_Primary_Functions_after.eps}
	        \caption{Impact of primary-to-backup capacity ratio}
	        \label{fig:p-bRatio}
        \end{figure}
\else
\afterpage{
    \vspace*{\fill}{
        \begin{figure}[h]
	        \vspace{-2mm}
	        \centering
		    \epsfig{width=4in,file=Percentage_of_Piggybacked_Functions_zoom.eps}
	        \caption{Impact of number of chains and backup capacity}
	        \label{fig:chain-cap}
        \end{figure}
        \begin{figure}[h]
	        \vspace{-2mm}
	        \centering
		    \epsfig{width=4in,file=Impact_of_Number_of_Primary_Functions_after.eps}
	        \caption{Impact of primary-to-backup capacity
			ratio}
	        \label{fig:p-bRatio}
        \end{figure}
    }
    \vspace*{\fill}
    \clearpage
}
\fi

Fig.~\ref{fig:chain-cap} summarizes the piggybacking percentage for
various numbers of chains and backup capacity. The primary capacity of
each server is fixed to 8. The figure shows a similar trend, in which
the piggybacking opportunities can be mostly utilized when the backup
capacity grows above 3, regardless off the number of chains in the
network.  Even if each server can only install two backup instances,
\name\ can still allow more than 93\% of instances to piggyback their
updates.  We next fix the total capacity of each server, but change
the ratio of resources allocated to primary and backup instances.  For
example, a 3:1 ratio implies that, in a server, 75\% of instances are
primary instances, while 25\% are backup instances.
Fig.~\ref{fig:p-bRatio} shows the percentage of piggybackable
instances as the primary capacity varies from 8 to 16.  The results
demonstrate that the piggybacking opportunities are closely related to
how much percentage of server resources is used for backup. If servers
reserve fewer resources for backup, the piggybacking opportunities
degrade. Resource allocation for primary and backup instance
deployment is an interesting issue worth future studies.


\ifx\isthesis\undefined
\begin{figure}[t!]
	\centering
	\epsfig{width=2.7in,file=Impact_of_Backup_Capacity.eps}
	\caption{Impact of backup-primary association limit (P:B capacity =
	2:1)}
	\label{fig:impactK}
\end{figure}

\begin{figure}[t!]
	\centering
	\epsfig{width=2.7in,file=Impact_of_Number_of_Primary_Functions_before.eps}
	\caption{Impact of backup-primary association limit (Backup capacity
	= 3)}
	\label{fig:impactK2}
\end{figure}
\else
\afterpage{
	\vspace*{\fill}{
		\begin{figure}[h!]
			\centering
			\epsfig{width=4in,file=Impact_of_Backup_Capacity.eps}
			\caption{Impact of backup-primary association limit
			(Primary:Backup capacity = 2:1)}
			\label{fig:impactK}
		\end{figure}

		\begin{figure}[h!]
			\centering
			\epsfig{width=4in,file=Impact_of_Number_of_Primary_Functions_before.eps}
			\caption{Impact of  backup-primary association limit (Backup
			capacity = 3)}
			\label{fig:impactK2}
		\end{figure}
		}
		\vspace*{\fill}
		\clearpage
	}
	\fi

\subsecc{Impact of Backup-Primary Association Limit}%Fig 11
We then check how the performance changes with the value of $K$
(maximal number of primary instances that can be associated with a
backup instance).  We try two different configurations. In
Fig.~\ref{fig:impactK}, we fix the ratio of primary capacity to backup
capacity per server to 2:1, while in Fig.~\ref{fig:impactK2}, we fix
the back capacity to 3 but vary the primary capacity from 6 to 14.
Recall that a smaller $K$ means that each backup instance can only
serve fewer primary instances. That is, the degree of competition
among primary instances becomes more severe when the system is short
of backup instances. The figures confirm again that the piggybacking
opportunities decrease as $K$ gets smaller.

Fig.~\ref{fig:impactK} shows that, when the overall capacity per
server is small, e.g., 6 primary instances per server, only a few
backup instances are deployed and the piggybacking opportunities
become small since fewer chains can traverse through a limited number
of backup instances. Similarly, given a fixed number of backup
instances, as in Fig.~\ref{fig:impactK2}, an increasing number of
primary instances leads to more severe competition, as a result making
some primary instances not be able to find any piggybackable chains.
The results reveal that piggybacking opportunities not only depend on
the number of chains but also the number of back instances distributed
in the network.

\ifx\isthesis\undefined
        \begin{figure}[t]
	        \centering
		    \epsfig{width=2.7in,file=Impact_of_Piggybacking_Chain.eps}
	        \caption{Effectiveness of chain selection}
	        \label{fig:chainselection}
        \end{figure}
        \begin{figure}[t]
	        \centering
		    \epsfig{width=2.7in,file=Performance_of_Shortest_Path.eps}
	        \caption{Performance of stand-alone instance deployment}
	        \label{fig:stand-alone}
        \end{figure}
\else

\afterpage{
    \vspace*{\fill}{
        \begin{figure}[h]
	        \centering
		    \epsfig{width=4in,file=Impact_of_Piggybacking_Chain.eps}
	        \caption{Effectiveness of chain selection}
	        \label{fig:chainselection}
        \end{figure}
        \begin{figure}[h]
	        \centering
		    \epsfig{width=4in,file=Performance_of_Shortest_Path.eps}
	        \caption{Performance of stand-alone instance deployment}
	        \label{fig:stand-alone}
        \end{figure}
    }
    \vspace*{\fill}
    \clearpage
}
\fi


\subsecc{Effectiveness of Chain Selection}%Fig 11
We next check whether our chain selection design can effectively
reduce the piggybacking cost as the mean packet arrival rate is
configured to 1 and 2 packets per millisecond, respectively.  We also
compare our chain selection with na\"{\i}ve FCFS. The results
illustrated in Fig.~\ref{fig:chainselection} show that FCFS introduces
a much higher piggybacking hop count since primary functions are more
likely to piggyback the update states in a chain traversing along a
long path.  With our arrival prediction, we try to embed the updates
in shorter chains if possible, as a result reducing the hop count by
around 27.5\% and 39.35\% with respect to the packet arrival rate of 1
and 2 packets per millisecond, respectively. The figure also shows
that a higher traffic rate increases the probability of identifying a
short piggybacking chain and results in a smaller piggybacking cost.

\subsecc{Performance of Stand-Alone Backup}%Fig 11
Finally, Fig.~\ref{fig:stand-alone} compares the backup hop count of
\name's cooperative stand-alone instance deployment and na\"{\i}ve
shortest path based deployment. The results show that the stand-alone
cost increases as the number of primary instances per server increases
due to a limited number of chains and, thus, limited piggybacking
opportunities.  By explicitly controlling the backup placement order
of prioritized primary instances, we can better utilize the remaining
available resources to reduce the cost of non-piggybackable primary
instances, as compared to the simple shortest path based scheme. The
gap between the two solutions grows as a network has more primary
instances, which should compete for limited backup capacity. Recall
the results shown in Fig.~\ref{fig:chainNum}(c). The reduced overall
update cost in terms of update bytes is also contributed by a more
efficient cooperative stand-alone instance deployment scheme of \name.




==> evaluation-2.tex <==
\ifx\isthesis\undefined
\begin{table}[t]
\small
\caption{Simulation Setups}
%\vspace{5mm}
\centering  \label{tab:Parameter}
\begin{tabular}{ll}
\toprule
Parameter         & Default configuration  \\
\toprule
Number of servers &20\\
Number of function types      & 20 \\
Number of chains      & 50 \\
Primary capacity & 8 \\
Backup capacity & 3 \\
Max backup-primary association ($K$) & 5\\
\bottomrule
\end{tabular}
\label{tb:setting}
\end{table}
\else
\afterpage{
\vspace*{\fill}{
\begin{table}[ht]
\small
\caption{List of Settings}
%\vspace{5mm}
\centering  \label{tab:Parameter}
\begin{tabular}{ll}
\toprule
Parameter         & Default configuration  \\
\toprule
Number of servers &20\\
Number of function types      & 20 \\
Number of chains      & 50 \\
Primary capacity & 8 \\
Backup capacity & 3 \\
Max backup-primary association ($K$) & 5\\
\bottomrule
\end{tabular}
\label{tb:setting}
\end{table}
}
\vspace*{\fill}
\clearpage
}
\fi

\secc{Performance Evaluation}\label{sec:results}
We conduct extensive simulations to evaluate the performance of \name\
in a fat tree topology~\cite{AlFares2008}, which has been widely used
in many data center networks. We deploy a 4-pods fat tree, which
consists of 16 hosts and three layers of switches, i.e., 8 edge
switches, 8 aggregation switches and 4 core switches.  Each switch
connects to a physical machine, which installs a number of VMs.
Without otherwise stated, the default number of function types and
chains are set to 20 and 50, respectively, and the maximal number of
primary instances and backup instances that can be installed in a
server (i.e., server capacity) is 8 and 3, respectively.  We assign
each primary instance to a randomly-selected physical machine. For
each function type, we randomly deploy a roughly equal number of
instances in the network until the capacity of all the servers has
been fully utilized. Each backup instance can be associated with up to
$K=5$ primary instances by default.  The packet size of each piggyback
update and stand-alone update, respectively, is set to 20 and 60
bytes.  The default parameter settings are summarized in
Table~\ref{tb:setting}.
%\del{\textblue{The default parameter settings are summarized in

\ifx\isthesis\undefined
\begin{figure*}[t]
\centering
\begin{tabular}{ccc}
\hspace{-12pt}
\epsfig{width=2.25in,file=Impact_of_Backup_Capacity_10.eps}&
\hspace{-10pt}
\epsfig{width=2.25in,file=Impact_of_Backup_Capacity_20.eps}&
\hspace{-10pt}
\epsfig{width=2.25in,file=Impact_of_Backup_Capacity_30.eps}\\
\footnotesize{(a) 10 chains}&
\footnotesize{(b) 20 chains }&
\footnotesize{(c) 30 chains }
\end{tabular}
\caption{Impact of backup capacity.}
\label{fig:capacity}
\end{figure*}
\else
\afterpage{
\vspace*{\fill}{
\begin{figure}[ht]
\centering
\begin{tabular}{c}
\epsfig{width=2.9in,file=Impact_of_Backup_Capacity_10.eps}\\
\footnotesize{(a) 10 chains}\\
\\
\epsfig{width=2.9in,file=Impact_of_Backup_Capacity_20.eps}\\
\footnotesize{(b) 20 chains }\\
\\
\epsfig{width=2.9in,file=Impact_of_Backup_Capacity_30.eps}\\
\footnotesize{(c) 30 chains }
\end{tabular}
\caption{Impact of backup capacity.}
\label{fig:capacity}
\end{figure}
}
\vspace*{\fill}
\clearpage
}
\fi

We generate a set of chains, each of which is from a random
originating host to a random destination host and requests a sequence
of NFs randomly selected from a set of function types $\mathcal{F}$.
The length of a chain is also picked randomly, varying from 1 to 20.
We leverage a simple closest instance assignment scheme to assign
primary instances to a chain. That is, for a chain requesting NF
$f_i\rightarrow f_{i+1}$ in steps $i$ and $i+1$, the instance of $f_i$
will forward this chain to the closest instance of $f_{i+1}$. The
traffic arrival pattern of each chain follows a Poisson process with
the mean arrival rate of 1 packet per millisecond. Since our goal is
to demonstrate the benefit of reusing SFCs, the primary instance
assignment for SFCs should not affect the performance much.

We compare \name\ with two baseline algorithms: {\em i) random
placement}, which deploys backup instances in randomly selected
servers without considering the locations of primary instances, and
{\em ii) shortest path based placement:} primary instances
sequentially pick the closest available servers to deploy (or reuse)
their backup instances, while the selection order of primary instances
is determined randomly.  Our evaluation will examine the impact of
number of chains, the impact of server capacity, the impact of
backup-primary association limit, the effectiveness of chain
selection, and the performance of stand-alone backup instance
placement.

\ifx\isthesis\undefined
\begin{figure}[t]
\centering
\epsfig{width=2.7in,file=Percentage_of_Piggybacked_Functions_zoom.eps}
\caption{Impact of number of chains and backup capacity}
\label{fig:chain-cap}
\end{figure}
\else
%
\fi

\subsecc{Impact of Number of Chains}%Fig 4,5,6
We first check the percentage of primary instances whose backup can be
piggybacked in the three comparison schemes.
Fig.~\ref{fig:chainNum}(a) shows the results when the number of chains
varies from 10 to 50. The figure shows that, as the number of chains
increases, the opportunities of piggybacking grow accordingly,
matching the intuition of our design.  Since our design explicitly
considers the locations of primary instances and the traversing paths
of chains, we can fully utilize the piggybacking opportunities and
obtain almost 100\% of piggybackable instances. However, random
placement and shortest path based deployment would underutilize the
opportunities as they do not consider the routing of chains.

Fig. \ref{fig:chainNum}(b) demonstrates the piggybacking hop counts of
the comparison methods. The results show that random placement does
not consider the locations of primary instances and, thus, lead to long
piggybacking paths.  Shortest path based placement achieves the minimal
piggybacking hop counts since it always deploys the backup instances
nearby the primary instances. However, as shown in
Fig.~\ref{fig:chainNum}(a), it supports piggybacking for only
40\%--60\% of primary instances. Hence, those non-piggybackable
instances still need to use stand-alone packets to deliver updates, as
a result increasing the overall cost. By contrast, \name\ allows
almost all the primary instances to piggyback their updates, through a
slightly longer path.

We then plot in Fig.~\ref{fig:chainNum}(c) the total number of update
bytes, including piggybacking and stand-alone packets, of the three
methods. The results verify that shortest path based placement sends
stand-alone updates for a large proportion of primary instances and,
overall, produces a significantly higher update overhead.  Though our
piggybacking updates traverse through slightly longer paths, the
average overall overhead can still be reduced by 39.56\%, as compared
to shortest path based placement, since we fully utilize piggybacking
opportunities and minimize the stand-alone update cost.

\subsecc{Impact of Server Capacity}%Fig 4,5,6
In this simulation, we examine the impact of backup capacity of each
server.  Figs.~\ref{fig:capacity}(a,b,c) illustrate the percentage of
piggybackable instances as the network includes 10, 20, and 30 chains,
respectively. For each figure, we plot the results when the backup
capacity varies from 2 to 6.  The results show that, when the backup
capacity increases, the piggybacking opportunities grow accordingly.
The percentage converges when the backup capacity increases to 4,
showing that a finite backup capacity can already ensure full
piggybacking updates. When the backup capacity is large enough, the
performance of various numbers of chains becomes indifferent. This
explains that, when a system supports sufficient backup capacity, even
a small number of chains can already realize the benefits of
piggybacking.

\ifx\isthesis\undefined
\begin{figure}[t]
\centering
\epsfig{width=2.7in,file=Impact_of_Number_of_Primary_Functions_after.eps}
\caption{Impact of primary-to-backup capacity ratio}
\label{fig:p-bRatio}
\end{figure}
\else
\begin{figure}[ht]
\vspace{-2mm}
\centering
\epsfig{width=3.7in,file=Impact_of_Number_of_Primary_Functions_after.eps}
\caption{Impact of primary-to-backup capacity
ratio}
\label{fig:p-bRatio}
\end{figure}
}
\vspace*{\fill}
\clearpage
}
\fi

Fig.~\ref{fig:chain-cap} summarizes the piggybacking percentage for
various numbers of chains and backup capacity. The primary capacity of
each server is fixed to 8. The figure shows a similar trend, in which
the piggybacking opportunities can be mostly utilized when the backup
capacity grows above 3, regardless off the number of chains in the
network.  Even if each server can only install two backup instances,
\name\ can still allow more than 93\% of instances to piggyback their
updates.  We next fix the total capacity of each server, but change
the ratio of resources allocated to primary and backup instances.  For
example, a 3:1 ratio implies that, in a server, 75\% of instances are
primary instances, while 25\% are backup instances.
Fig.~\ref{fig:p-bRatio} shows the percentage of piggybackable
instances as the primary capacity varies from 8 to 16.  The results
demonstrate that the piggybacking opportunities are closely related to
how much percentage of server resources is used for backup. If servers
reserve fewer resources for backup, the piggybacking opportunities
degrade. Resource allocation for primary and backup instance
deployment is an interesting issue worth future studies.


\ifx\isthesis\undefined
\begin{figure}[t!]
\centering
\begin{tabular}{c}
\epsfig{width=2.7in,file=Impact_of_Backup_Capacity.eps}\\
\footnotesize{(a) Primary:Backup capacity = 2:1}\\
\\
\epsfig{width=2.7in,file=Impact_of_Number_of_Primary_Functions_before.eps}\\
\footnotesize{(b) Backup capacity = 3 }
\end{tabular}
\caption{Impact of maximal number of back-primary
association}
\label{fig:impactK}
\end{figure}
\else
\afterpage{
\vspace*{\fill}{
\begin{figure}[h!]
\centering
\epsfig{width=4in,file=Impact_of_Backup_Capacity.eps}
\caption{Impact of maximal number of back-primary
association (Primary:Backup capacity = 2:1)}
\label{fig:impactK}
\end{figure}

\begin{figure}[h!]
\centering
\epsfig{width=4in,file=Impact_of_Number_of_Primary_Functions_before.eps}
\caption{Impact of maximal number of back-primary
association (Backup capacity = 3)}
\label{fig:impactK2}
\end{figure}
}
\vspace*{\fill}
\clearpage
}

\fi

\subsecc{Impact of Backup-Primary Association Limit}%Fig 11
We then check how the performance changes with the value of $K$
(maximal number of primary instances that can be associated with a
backup instance).  We try two different configurations. In
Fig.~\ref{fig:impactK}, we fix the ratio of primary capacity to backup
capacity per server to 2:1, while in Fig.~\ref{fig:impactK2}, we fix
the back capacity to 3 but vary the primary capacity from 6 to 14.
Recall that a smaller $K$ means that each backup instance can only
serve fewer primary instances. That is, the degree of competition
among primary instances becomes more severe when the system is short
of backup instances. The figures confirm again that the piggybacking
opportunities decrease as $K$ gets smaller.

Fig.~\ref{fig:impactK} shows that, when the overall capacity per
server is small, e.g., 6 primary instances per server, only a few
backup instances are deployed and the piggybacking opportunities
become small since fewer chains can traverse through a limited number
of backup instances. Similarly, given a fixed number of backup
instances, as in Fig.~\ref{fig:impactK2}, an increasing number of
primary instances leads to more severe competition, as a result making
some primary instances not be able to find any piggybackable chains.
The results reveal that piggybacking opportunities not only depend on
the number of chains but also the number of back instances distributed
in the network.

\ifx\isthesis\undefined
\begin{figure}[t]
\centering
\epsfig{width=2.7in,file=Impact_of_Piggybacking_Chain.eps}
\caption{Effectiveness of chain selection}
\label{fig:chainselection}
\end{figure}
\begin{figure}[t]
\centering
\epsfig{width=2.7in,file=Performance_of_Shortest_Path.eps}
\caption{Performance of stand-alone instance deployment}
\label{fig:stand-alone}
\end{figure}

\begin{figure}[ht]
\centering
\epsfig{width=2.7in,file= Success.eps}
\caption{Chain selection success probability}
\label{fig:successprob}
\end{figure}
\else

\afterpage{
\vspace*{\fill}{
\begin{figure}[t]
\centering
\epsfig{width=3.7in,file=Impact_of_Piggybacking_Chain.eps}
\caption{Effectiveness of chain selection}
\label{fig:chainselection}
\end{figure}
\begin{figure}[ht]
\vspace{-2mm}
\centering
\epsfig{width=3.7in,file=Performance_of_Shortest_Path.eps}
\caption{Performance of stand-alone instance deployment}
\label{fig:stand-alone}
\end{figure}
}
\vspace*{\fill}
\clearpage
}
\fi

\afterpage{
\vspace*{\fill}{
\begin{figure}[ht]
\centering
\begin{tabular}{c}
\epsfig{width=2.8in,file=Dense_sparse_pg_ratio.eps}\\
(a) percentage of piggybackable instances \\
\epsfig{width=2.8in,file=Dense_Sparse_Hop_counts.eps}\\
(b) total number of hop counts\\
\epsfig{width=2.8in,file=Dense_sparse_update_bytes.eps}\\
(c) total size of updates
\end{tabular}
\caption{Impact of topology.}
\label{fig:topology}
\end{figure}
}
\vspace*{\fill}
\clearpage
}


\subsecc{Effectiveness of Chain Selection}%Fig 11
We next check whether our chain selection design can effectively
reduce the piggybacking cost as the mean packet arrival rate is
configured to 1 and 2 packets per millisecond, respectively.  We also
compare our chain selection with na\"{\i}ve FCFS. The results
illustrated in Fig.~\ref{fig:chainselection} show that FCFS introduces
a much higher piggybacking hop count since primary functions are more
likely to piggyback the update states in a chain traversing along a
long path.  With our arrival prediction, we try to embed the updates
in shorter chains if possible, as a result reducing the hop count by
around 27.5\% and 39.35\% with respect to the packet arrival rate of 1
and 2 packets per millisecond, respectively. The figure also shows
that a higher traffic rate increases the probability of identifying a
short piggybacking chain and results in a smaller piggybacking cost.

We further plot the success probability of chain selection in
Fig.~\ref{fig:successprob} when the packet arrival rate is configured
to 1 and 2 packets per millisecond, respectively. The results show
that, when the packet arrival rate is sufficiently high (2 packets per
ms), over 80\% of our prediction can correctly identify the arrival
events of the candidate chain, which reduces the forwarding latency
effectively. Even for a lower arrival rate (1 packet per ms), we can
still identify the candidate with a probability of around 60\%--70\%.
The lower probability is due to the few arrival events. Overall, we can
conclude that, with arrival prediction, each primary function can have
a fairly high opportunity to piggyback the update information in a
short chain and, thus, reduce the update cost.

\subsecc{Impact of Topology}
We next check the impact of network topology on the update costs.
\textblue{In this simulation, we deploy 20 servers, but connect any
two servers with a random probability, following the discrete uniform distribution.
To tune the density of a network, we change the mean connection
probability to 80\% and 20\%, which simulate a dense and sparse network,
respectively.} Fig.~\ref{fig:topology}(a) shows that the piggyback
ratio of sparse graph is higher in a sparse graph. The reason is that,
when a network is sparse, SFCs only have a few available paths and
need to go through more network links, which hence increases the
probability of traversing through multiple primary instances and
backup instances.  This can also be observed in
Fig.~\ref{fig:topology}(b), which illustrates that the piggybacking
path in a sparse graph is far more than that in a dense graph.
Finally, Fig.~\ref{fig:topology}(c) indicates that, though a dense
graph has fewer piggybacking opportunities, it has more links and
usually results in a shorter forwarding path. Hence, the overall
update cost of a dense graph is much lower than that of a sparse
graph.


\subsecc{Performance of Stand-Alone Backup}%Fig 11
Finally, Fig.~\ref{fig:stand-alone} compares the backup hop count of
\name's cooperative stand-alone instance deployment and na\"{\i}ve
shortest path based deployment. The results show that the stand-alone
cost increases as the number of primary instances per server increases
due to a limited number of chains and, thus, limited piggybacking
opportunities.  By explicitly controlling the backup placement order
of prioritized primary instances, we can better utilize the remaining
available resources to reduce the cost of non-piggybackable primary
instances, as compared to the simple shortest path based scheme. The
gap between the two solutions grows as a network has more primary
instances, which should compete for limited backup capacity. Recall
the results shown in Fig.~\ref{fig:chainNum}(c). The reduced overall
update cost in terms of update bytes is also contributed by a more
efficient cooperative stand-alone instance deployment scheme of \name.






==> intro-1.tex <==
\secc{Introduction}
Network functions (NFs) typically provide network services such as as
load balancers, firewalls, network address translation (NAT), and deep
packet inspection in a network. Conventionally, those services can
only be implemented in specific hardware. However, with the emergence
of software-defined networks, it has become flexible and efficient to
support software-based services in virtual machines (VMs), which is
known as {\em network function virtualization} (NFV). The design of
NFV enables network operators to install virtualized NFs according to
dynamic demands and provide clients customized service by flexible
{\em service function chaining} (SFC).

For a network enabling NFV, system reliability is of importance since
virtual machines are prone to errors and recovering virtual NFs
usually takes non-negligible latency~\cite{xx}.  Hence, providing
fault tolerance is essential for an NFV-enabled SDN.  Conventional
fault tolerance designs usually enhance reliability by introducing
redundancy~\cite{xxx,yyy}. In particular, to ensure reliability of a
network function, one can deploy a primary NF instance in a VM and
further install a redundant NF instance as a backup in a different VM.
Alternatively, two NF instances can be installed in different VMs,
both used to service their own clients and, at the same time, acting
as the backup of each other.  This type of fault tolerance is called
{\em active-active} backup as both the primary and redundant NF
instances are active.

However, for active-active backup, primary and redundant NF instances
usually operate independently and do not synchronize their states.
That is, the states will not be consistent when services are migrated
to redundant instances due to the failure of their primary NF
instances.  For instance, a service may have been authorized by its
primary NF instance to access a private database, but is rejected by
its backup instance as the verification information is not known by
the backup.  To resolve this limitation, an alternative, called {\em
active-standby} backup, has been proposed to allow a backup to only
keep the state information of primary NF instances but do not actually
serve clients. Those standby backup instances can be activated
immediately with the up-to-date states once their primary instances
fail.

Recent efforts~\cite{xxx} have investigated an efficient and
light-weight scheme to launch standby backup instances. However, an
open problem still remains unsolved: {\em efficient state update}.  To
ensure state consistency, each stateful primary instance should
periodically forward state information to its corresponding backup
instance.  Those periodical state update would incur tremendous
traffic load. We notice that the update cost closely depends on the
location of primary and backup instances. Intuitively, we can reduce
the update cost by installing a backup instance close to its primary
instance. However, as the computing resources in a network are
limited, a backup instance may have to serve multiple primary
instances, which compete with each other.  Hence, our goal is to
investigate an efficient backup instance deployment and update
protocol so as to minimize the overall state update cost. 

\begin{figure}[tb]
    \centering
    \includegraphics[scale=0.4]{fig/fig1.eps}
    \caption{Reuse existing SFCs to piggyback backup updates}
    \label{fig:1}
\end{figure}

In this paper, we propose an efficient backup instance deployment and
update protocol, called \name\ ({\em Piggyback-based Backup}).  Our
design is motivated by a key observation: {\em an SDN has typically
served a large number of service function chains that traverse through
diverse routes and can help piggyback the backup update information.}
As state updates usually generate periodical but small packets, the
headers of those small update packets become the major overhead of
state update. By piggybacking the state information in existing SFCs,
we can significantly reduce the update cost, as illustrated in
Fig.~\ref{fig:1}.

To realize this idea, we have to address two practical challenges.
First, to enable piggybacking, the backup instance should be deployed
in a VM traversed by existing SFCs who have passed through its primary
instances.  We call those back instances {\em piggybackable backup
instances}, e.g., XXX in Fig.~\ref{fig:xxx}. Though there may exist
several chains that traverse through a primary instance and can help
piggyback the backup information, their routing paths, however, have
already been assigned based on their customized demands. Hence, the
cost of information update does not depend on the distance between the
primary instance and backup instance anymore, but is determined by the
routing length of piggybacking chains from a primary instance to its
backup instance.  Backup instances should now be deployed according to
the distribution of existing service chains. Second, since many SFCs
can be candidates to piggyback the update information, the one with a
shorter piggybacking path should be preferable. However, as traffic
arrivals of a SFC is unpredictable, selecting proper chains to
piggyback the updates becomes difficult. Finally, as the VM resources
are limited and the distribution of SFCs cannot be controlled, some
primary NF instances may not have any chance to piggyback their update,
e.g., NF E in node 6 in Fig.~\ref{fig:1}.  Their update can only be
forwarded as stand-alone packets. 

To address those challenges, we develop a backup instance deployment
algorithm that enhances the opportunities of update piggybacking and
minimize the cost of stand-alone updates. We then propose a chain
selection scheme based on chain arrival prediction to reduce the
piggybacking cost.  We conduct extensive simulations to verify the
effectiveness of our design.  The simulation results show that \name\
outperforms both random deployment and shortest path first deployment
by 40-50\% in terms of the overall update load.

The rest of the \article\ is organized as follows.
\sect~\ref{sec:related} reviews recent work on VNF fault tolerance
designs and NF deployment. \sect~\ref{sec:problem} formally defines
the backup instance deployment problem, and \sect~\ref{sec:design}
elaborates the design of \name. We evaluate the performance in
\sect~\ref{sec:results}, and conclude this work in
\sect~\ref{sec:conclusion}.


==> related-thesis.tex <==
\section{Background and Related Work}

\subsection{Background}
Software Defined Network (SDN) is a new network architecture that
separates the control plane and data plane from routers. In SDN, the
network functions (NFs), such as firewall, network address translation
(NAT) and deep packet inspection (DPI) are usually virtualized, and it
is so called Network Function Virtualization (NFV). Different from the
traditional method, which makes the NFs embedded into dedicated
hardware that is costly and difficult to reconfigure, NFV provides
more flexible and inexpensive support of NFs. Those NFs can be
implemented as software running on virtual machines (VMs), which are
called, virtualized network functions (VNFs). The network request that
passes through several different VNFs is service function chain (SFC)
\cite{Ren2018}\cite{Ren2017}, because the network traffic may travel
through different VNFs, so we cannot just consider shortest path from
source to destination.

In order to achieve highly reliable SDN, we need to do some protection to stateful VNFs in case of failures. 


\subsection{Related Work}
Lots of studies have designed the highly available network systems \cite{Cully2008}\cite{Sherry2015}\cite{Rajagopalan2013}. Ref \cite{Cully2008} offered a checkpoint based fault tolerant network with three high-level goals, generality, transparency, and seamless failure recovery. Ref \cite{Rajagopalan2013} maintains the state of network flows by using light checkpoint, and it was the first fault tolerant system for VNFs.

In general, the existing work falls into three categories: hardware  \cite{Potharaju2013}, VNFs \cite{Chandrasekaran2016}, and software infrastructure \cite{Jacobson2014}\cite{Nobach2017}\cite{Stratus}. First, in hardware, it is the most traditional method; it has some advantages, however, the resource utilization is very low, about 50\%. Second, in VNFs, programmers need to write code for specific VNFs to protect their states. Ref \cite{Chandrasekaran2016} uses this method and leverages state transform technique to avert the need for manual intervention, however, it takes a long time to deploy. Third, in software infrastructure, it is the most commonly used method now. Ref \cite{Jacobson2014}\cite{Nobach2017} implements a robust system to do state transfer in SDN. Stratus technology \cite{Stratus} has developed a cloud solution to achieve state consistency on stateful VNFs, and our algorithm design is based on this solution.

 So far, there has been a large amount of research in VM deployment in clouds and data center networks \cite{Alicherry2012}\cite{Jayasinghe2011}\cite{Meng2010}.Ref \cite{Luizelli2015} proposed an integer linear programming model to solve the placement, assignment, and chaining problems. They first find a place to deploy the VNFs, and then assign them to network flow, finally generate paths to link those VNFs. However, it does not take VNF placement order into consideration. LightChain \cite{Hirwe2016} improves \cite{Luizelli2015} by leveraging topological sort to decide VNF placement order, and provides a primary function placement algorithm to optimize the number of switches between ingress and egress points of chains, reduce flow rules in switches, and eliminate Ping-Pong traffic, however, it doesn\textceltpal t have backup functions deployment, and resource usage doesn\textceltpal t take into consideration.In general, there are two modes of implementing state update: Active-Active mode\cite{Francisco2017}\cite{Carpio2017} and Active-Standby mode\cite{Jacobson2014}\cite{Nobach2017}\cite{Stratus}\cite{Kanizo2017}. Ref \cite{Francisco2017}\cite{Carpio2017} adopt Active-Active mode and develop LP model to optimize reliability and server usage, however, they do not discuss an important issue, state consistency. Ref \cite{Kanizo2017} adopts the same mode as ours, Active-Standby mode, and it converts the problem into graph theory to analyze, because of this, it sets lots of constraints, such as single primary function per VM and backup function cannot collocate with primary functions.



